When to intervene? Prescriptive Process Monitoring Under Uncertainty and Resource Constraints

Prescriptive process monitoring approaches leverage historical data to prescribe runtime interventions that will likely prevent negative case outcomes or improve a process's performance. A centerpiece of a prescriptive process monitoring method is its intervention policy: a decision function determining if and when to trigger an intervention on an ongoing case. Previous proposals in this field rely on intervention policies that consider only the current state of a given case. These approaches do not consider the tradeoff between triggering an intervention in the current state, given the level of uncertainty of the underlying predictive models, versus delaying the intervention to a later state. Moreover, they assume that a resource is always available to perform an intervention (infinite capacity). This paper addresses these gaps by introducing a prescriptive process monitoring method that filters and ranks ongoing cases based on prediction scores, prediction uncertainty, and causal effect of the intervention, and triggers interventions to maximize a gain function, considering the available resources. The proposal is evaluated using a real-life event log. The results show that the proposed method outperforms existing baselines regarding total gain.

==> BPM22_shoush/Abstract.tex <==
\begin{abstract} \label{sec:abstract}
Prescriptive process monitoring approaches leverage historical data to prescribe runtime interventions that will likely prevent negative case outcomes or improve a process’s performance. A centerpiece of a prescriptive process monitoring method is its intervention policy: a decision function determining if and when to trigger an intervention on an ongoing case. Previous proposals in this field rely on intervention policies that consider only the current state of a given case. These approaches do not consider the tradeoff between triggering an intervention in the current state, given the level of uncertainty of the underlying predictive models, versus delaying the intervention to a later state. Moreover, they assume that a resource is always available to perform an intervention (infinite capacity). This paper addresses these gaps by introducing a prescriptive process monitoring method that filters and ranks ongoing cases based on prediction scores, prediction uncertainty, and causal effect of the intervention, and triggers interventions to maximize a gain function, considering the available resources. The proposal is evaluated using a real-life event log. The results show that the proposed method outperforms existing baselines regarding total gain.

%Prescriptive process monitoring approaches leverage historical data to prescribe runtime interventions that are likely to prevent negative case outcomes or improve the process's performance. A centerpiece of a prescriptive process monitoring method is its intervention policy: a decision function that determines if and when to trigger an intervention on an ongoing case. Previous proposals in this field rely on intervention policies that consider only the current state of a case. These approaches do not consider the tradeoff between triggering an intervention in the current state, given the level of uncertainty of the underlying predictive models, versus delaying the intervention to a later state. Moreover, they assume that there is always a resource available to perform an intervention (infinite capacity).  This paper addresses these gaps by introducing a prescriptive process monitoring method that filters and ranks ongoing cases based on prediction scores, prediction uncertainty, and the causal effect of the intervention, and triggers interventions to maximize a gain function, considering the available resources. The proposal is evaluated using a real-life event log. The results show that the proposed method outperforms existing baselines in terms of net gain.

%The method uses an ensemble model to estimate the total uncertainty and probability of cases likely to end with unfavorable outcomes, in combination with a causal model to assess the influence of an intervention on cases' outcomes. 
%These estimates with a filtering and scoring method are embedded in a resource allocator that assigns resources to perform interventions to maximize an adjusted gain.
% that employ interventions are infinite. In practice, obtaining knowledge about the future state of ongoing cases from comparable prospective ones could support the proper allocation of resources to execute the preferred intervention to maximize payoff
%Existing techniques in this space consider only one or current state of ongoing business cases and trust in the predicted outcome. 
%However, they ignore quantifying the uncertainty attached to the predicted outcome or acquiring knowledge about what will happen to ongoing cases in the future state and comparing it to the current. 




%Prescriptive Process monitoring techniques aim to optimize business processes by prescribing how and when process workers intervene to preclude undesired measures of interest,e.g., outcome. Recent prescriptive process monitoring methods consider only the current state of ongoing business cases and trust in the predictive model's output regardless of measuring the uncertainty of the predictive model's outcome or considering that resources that employ interventions are finite. In practice,  Acquiring knowledge about present ongoing cases from comparable prospective ones could support the proper allocation of resources to execute the preferred intervention. This paper introduces a prescriptive monitoring technique that optimizes resource allocation to initiate interventions to optimize gain function. The approach depends on predictive modeling, estimating the uncertainty and probability of cases likely to end with adverse outcomes, in combination with a causal model to assess the influence of an intervention on cases' outcomes. These estimates with a technique to discover what will happen in the future are embedded in a resource allocator that assigns resources to interventions to maximize profit. Empirical results show.
\end{abstract}
\keywords{Prescriptive Process Monitoring \and Causal Inference \and Uncertainty}


==> BPM22_shoush/Approach.tex <==
\section{Approach} \label{sec:approach}

\begin{figure*}[!htb]
	\begin{center}
        \resizebox{\textwidth}{!}{\includegraphics{images/BPM_Approach6.pdf}}
		\caption{An overview of the proposed approach.}
		\label{fig:approach}
	\end{center}
\end{figure*}

The proposed PrPM method consists of two main phases, training and testing, see Fig.~\ref{fig:approach}. In the training phase, we train two ML models, i.e., predictive and causal. While in the testing phase, we present filtering and ranking techniques to determine the most profitable case. Then, decide when to trigger an intervention for the selected case to maximize a gain function—considering ongoing cases’ current and future state scores, uncertainty estimation, and resource availability.

%The proposed PrPM method consists of two main phases, training and testing, see Fig.~\ref{fig:approach}. The training phase train an ensemble and causal models to estimate the prediction scores and uncertainty. While the testing phase filters ongoing cases that are likely to end negatively into candidates, then rank them to select the most profitable one. Furthermore, determine when to trigger an intervention for the chosen case to maximize gain—considering ongoing cases’ current and future states scores, uncertainty estimation, and resource availability.





%The proposed PrPM method consists of two main phases, see Fig.~\ref{fig:approach}. Its primary objective is to filter negative ongoing cases into candidate cases, then rank them to select the best one. Furthermore, determine when to trigger an intervention for the best case to maximize an adjusted gain function—considering ongoing cases' current and future states, uncertainty estimation, and resource availability.

%Our PrPM method consists of two main phases, as shown in Fig. \ref{fig:approach}. Its primary objective is to pick among all candidate cases the best one to be treated and determine when to trigger an intervention, considering the current and future state of the process execution, uncertainty estimation, and resources availability.

% Our PrPM approach's main objective is to pick among all candidate cases the best one to be treated and to determine when to trigger an intervention, considering the current and following state of the process execution, uncertainty estimation, and resources availability.



%The approach consists of two main phases, as shown in Fig. \ref{fig:approach}. In the training phase, we construct an ensemble model to estimate the probability of cases that are likely to end with unfavorable outcomes, in addition to quantifying the uncertainty of its predictions. Additionally, we use a causal model from our recent work~\cite{shoush2021prescriptive} to estimate the intervention effect. In the testing phase, we introduce filtering and scoring methods to pick the most suitable case and assign it to a resource allocator from our previous work~\cite{shoush2021prescriptive}. 

% \begin{figure*}[!htb]
% 	\begin{center}
%         \resizebox{\textwidth}{!}{\includegraphics{images/pred_m.pdf}}
% 		\caption{Predictive}
% 		\label{fig:approach}
% 	\end{center}
% \end{figure*}

\subsection{Training Phase}
We first prepare the process execution data; then, we construct an ensemble-based predictive model to estimate the prediction scores, i.e., the probability of cases likely to end negatively and quantify the prediction uncertainty. Further, we build a causal model to estimate the $CATE$.



%We first prepare the process execution data; then, we construct an ensemble-based predictive model to estimate the prediction scores, i.e., probability of cases likely to end negatively, and quantify the prediction uncertainty. Further, we use a causal model developed in our recent work~\cite{shoush2021prescriptive} to estimate the $CATE$.

%We first prepare the event log; then, we construct an ensemble-based predictive model to estimate the probability of cases likely to end negatively and quantify the predictive uncertainty. Further, we use a causal model developed in our recent work~\cite{shoush2021prescriptive} to estimate the $CATE$. 

%In the training phase, we first prepare the process execution data; then, we construct an ensemble model to estimate the probability of cases that are likely to end with unfavorable outcomes, in addition to quantifying the uncertainty of its predictions. Further, we use a causal model from our recent work~\cite{shoush2021prescriptive} to estimate the intervention effect (or $CATE$).

% In the training phase, we construct an ensemble model to estimate the probability of cases that are likely to end with unfavorable outcomes, in addition to quantifying the uncertainty of its predictions. Additionally, we use a causal model from our recent work~\cite{shoush2021prescriptive} to estimate the intervention effect.


\subsubsection{Event Log Preprocessing}
This step is vital for PPM or PrPM tasks. In PPM, it includes \textit{data cleaning, prefix extraction, and prefix encoding} see Fig.~\ref{fig:pred}. These steps have been discussed in Teinemaa et al.~\cite{teinemaa2019outcome}, and we follow their suggestions here. We first pre-process the log to dismiss incomplete cases and then extract length $k$ from every case that results in a so-called \textit{prefix log}. This prefix extraction ensures that our training data is equivalent to the testing data. Finally, we encode each trace prefix into a feature vector ($X$) to train the predictive ensemble model, see Fig.~\ref{fig:pred}.

%to train the predictive ensemble model. 

%Finally, we encode the prefix log into a fixed-size \textit{feature vector} in order to be able to train the predictive ensemble model. 

\begin{figure*}[!htb]
	\begin{center}
        \resizebox{\textwidth}{!}{\includegraphics{images/pred_v5.pdf}}
		\caption{An overview of the ensemble model. }
		\label{fig:pred}
	\end{center}
\end{figure*}


While in PrPM, one further step is needed to analyze and understand the data and the business objective to identify an intervention $T$ that could positively impact an outcome $Y$. Moreover, determining what other variables ($W$: a.k.a. \textit{confounders}) affect the intervention and outcome. %Once the data is prepared, we train predictive and causal models.

%While in PrPM, one further step is needed to analyze and understand the data and the business objective. Consequently, identifying $T$ that could positively impact $Y$. Moreover, determining what other variables ($W$: aka \textit{confounders}) simultaneously affect the intervention and outcome. 

%Moreover, determining what other variables ($W$: aka \textit{confounders}) affect the intervention and the outcome simultaneously. 


%Event log preprocessing is crucial in the predictive (PPM) and prescriptive (PrPM) process monitoring tasks. In PPM tasks, generally, preprocessing step includes \textit{data cleaning, prefix log extraction, and prefix encoding} to have features vector $(X)$ in the correct format for building machine learning algorithms, as shown in Fig. \ref{fig:pred}. These steps have been discussed in Teinemaa et al. \cite{teinemaa2019outcome}, and we follow their suggestions n our work. 

%While in PrPM, the main task is to analyze and understand the data and the business objective to identify \textit{intervention} $(T)$ that could have an impact on the \textit{outcome} $(Y)$ and what other features ($W$: aka \textit{confounders}) that affect both the intervention and the outcome in the same time. 

\subsubsection{Ensemble model}
We construct an outcome-oriented predictive model (a classification problem from an ML perspective) via ensemble learning~\cite{dietterich2002ensemble}, as shown in Fig. \ref{fig:pred}. The principal assumption of ensemble learning is constructing one robust predictive model from several weak ones. Accordingly, the overall prediction scores performance would be superior where overfitting and the chance of getting a local minimum are avoided, which has two advantages to our work. First, it ensures  that we will accurately predict the probability of negative outcomes, i.e., \textit{the prediction score}. Second, it allows estimating \textit{the prediction uncertainty}.

% attached to each prediction. 

% We construct an outcome-oriented predictive model (a classification problem from ML perspective) via ensemble learning, as shown in Fig. \ref{fig:pred}., with two main objectives. First, to estimate the probability of cases leading to adverse outcomes. Second, to quantify the uncertainty of estimated probabilities.

% The principal assumption of ensemble learning is constructing one robust learner model from several weak ones. Accordingly, the overall prediction performance would be superior to one learner, which has two advantages in our work. First, it guarantees that we will predict the probability of unfavorable outcomes as accurately as possible. Second, it gives us the ability to estimate the uncertainty attached to each prediction. 

A single classifier in the ensemble is a  probabilistic model $cls_i: f(X, P_{uout_i})$. $X$ is the input feature vector, and the $P_{uout_i}$ is the estimated probability of cases likely to end with negative outcomes where $i \in \{1, m\}$, and $m$ is the number of classifiers in the ensemble. We then define the \textit{prediction score} as the average of individual classifiers’ prediction scores $(avg_{pred})$, as shown in Eq.~\ref{eq:avgpred}. The following step is to estimate the prediction uncertainty.% attached to the $avg_{pred}$.

%\begin{definition}{\textit{\textbf{Classifier.}}} A classifier $cls_i: f(X, P_{uout_i})$ is a probabilistic learner that takes a feature vector $X$ as input to estimate the probability of undesired outcomes $P_{uout_i}$, where $i \in \{1, m\}$, and $m$ is the number of classifiers in the ensemble. 
%\end{definition}
% We take the mean prediction from all learners to estimate the probability of cases likely to end with adverse outcomes ($avg_{pred}$) from the ensemble model. 

%We define the probability of cases likely to end with adverse outcomes as the average of individual learners' probabilities obtained from different learners in the ensemble.
% We define the probability of cases likely to end with adverse outcomes from the ensemble model as the average of individual learners' predictions ($avg_{pred}$).
%We define the probability of cases likely to end with adverse outcomes from the ensemble model as the average of individual learners' predictions,

%We define the probability of cases likely to end negatively as the average of individual learners' predictions $(avg_{pred})$, as shown in Eq. \ref{eq:avgpred}. The following step is to estimate the uncertainty attached to the  $avg_{pred}$. 

%We define the probability of cases likely to end with adverse outcomes as the average of individual learners' probabilities obtained from different learners in the ensemble $(avg_{pred})$, as shown in Eq. \ref{eq:avgpred}. The following step is to estimate the uncertainty attached to the average prediction. 

	\begin{equation}
	avg_{pred} = \frac{\sum_{i=1}^{m}P_{uout_i}}{m}
        % gain(c_{id}, T_{i=1}) = cost(c_{id}, T_0)  - cost(c_{id}, T_{i=1})
        \label{eq:avgpred}
    \end{equation}
    
There are two sources of uncertainties where predictive models become unsure about predictions~\cite{hullermeier2021aleatoric}. The first source is \textit{data (or aleatoric)} uncertainty $(\sigma)$. It is a property of the distribution that generates cases, and it occurs when \textit{outcomes overlap} or there is \textit{noise} in the underlying data distribution. The second source is \textit{knowledge (or epistemic)} uncertainty $(\rho)$. It is a property of the predictive model's learning parameters and arises due to a lack of model knowledge. It appears when there is \textit{out-of-distribution} input. Both sources form the prediction uncertainty, i.e., \textit{total uncertainty} ($total_{uncer}$), see Eq.~\ref{eq:tuncer1}.

%\textit{total uncertainty} ($total_{uncer}$), as shown in Eq.~\ref{eq:tuncer1}.
    
%There are two types of uncertainties in the context of predictive models to measure how the models are sure about their predictions~\cite{hullermeier2021aleatoric}. First, \textit{data (or aleatoric)} uncertainty $(\sigma)$ is a property of the distribution that yielded the samples to measure noise. Second, \textit{knowledge (or epistemic)} uncertainty $(\rho)$, i.e., a property of the model's parameters that deal with out-of-distribution data. Both types are added to form \textit{total uncertainty}, as shown in Eq. \ref{eq:tuncer1}. 

	\begin{equation}
	total_{uncer} = \sigma + \rho
	\label{eq:tuncer1}
    \end{equation}
    
    
The proper level of $\sigma$ is defined as \textit{entropy} of the actual underlying data distribution~\cite{malinin2020uncertainty}. Here, the entropy is the average level of surprise or uncertainty inherent in the possible outcomes. It is calculated for a random variable $S$ with $c$ in $C$ discrete states, see Eq.~\ref{eq:entropy}, where $P(c)$ is the probability of $c$ to occur. 

	\begin{equation}
	Entropy(S) = - {\sum_{c \in C} P(c)\log(P(c)}
	\label{eq:entropy}
    \end{equation}

However, we do not have access to the actual underlying data distribution, but our model is probabilistic and is trained on this data. So measuring the entropy of our probabilistic model, i.e., trained using \textit{negative log-likelihood}, estimates the level of $\sigma$. In particular, we obtain a distribution over outcome labels from individual classifiers in the ensemble for a given case, and $\sigma$ is the average \textit{entropy} of the individual prediction scores, as shown in Eq.~\ref{eq:duncer}.%, where $P(c)$ is the probability of $c$ state to occur.
    
%For example, we get a distribution over outcome labels for a particular case, and the $\sigma$ is estimated as the \textit{entropy} of that distribution, as shown in Eq.~\ref{eq:duncer}.


%A proper estimate of the data uncertainty is defined as the \textit{entropy} of the underlying distribution~\cite{malinin2020uncertainty}. We define entropy as the average level of surprise or uncertainty inherent in the possible outcomes to estimate models' uncertainties. However, we do not have access to the underlying data distribution, but our model is probabilistic and is trained on this data. So measuring the entropy of our probabilistic model, i.e., trained using maximum likelihood estimation, gives us an estimate of the level of data uncertainty. For example, we get a distribution over outcome labels for a particular case, and the data uncertainty is the average entropy over that distribution, as shown in Eq. \ref{eq:duncer}.

	\begin{equation}
	\sigma = \frac{\sum_{i=1}^{m}Entropy(P_{uout_i})}{m}
        % gain(c_{id}, T_{i=1}) = cost(c_{id}, T_0)  - cost(c_{id}, T_{i=1})
        \label{eq:duncer}
    \end{equation}

Furthermore, we rely on the \textit{Bayes rule}~\cite{stone2013bayes} to estimate the $\rho$~\cite{malinin2020uncertainty}. Assume we obtain a posterior over model parameters that give us the distribution over likely models that have generated the data. Accordingly, models sampled from the obtained distribution agree on data they have seen and provide similar predictions, indicating low $\rho$. However, if the models do not understand the input, they provide diverse predictions and strongly disagree, indicating high $\rho$. Thus, $\rho$ is the mutual information between the models' parameters and the predictions. 

%We take the difference between $total_{uncer}$ and $\sigma$ to quantify the $\rho$. 

%On the other hand, we require an ensemble of probabilistic models to estimate knowledge uncertainty defining the lack of training data~\cite{malinin2020uncertainty}. Based on the \textit{Bayes rule}, assume we obtain a posterior over model parameters, which give us the distribution over likely models that have generated the data we have seen. Accordingly, models sampled from the obtained distribution should agree on data they have seen and give similar predictions, indicating low $\rho$. However, if the models do not understand the input, they are likely to provide diverse predictions and strongly disagree, indicating high $\rho$.

%On the other hand, we require an ensemble of probabilistic models to estimate the knowledge uncertainty defining the lack of training data~\cite{malinin2020uncertainty}. Based on the \textit{Bayes rule}, assume we obtained a posterior over model parameters which give us the distribution over likely models which have generated the data we have seen. Accordingly, models sampled from the obtained distribution should agree on data they have seen and give similar predictions, which means low knowledge uncertainty. However, if the models do not understand the input, they are likely to provide diverse predictions and strongly disagree, indicating high knowledge uncertainty.

Similarly, the total uncertainty is the entropy of the average prediction, see Eq.~\ref{eq:tuncer2}. To exemplify the estimation of the prediction uncertainty ($total_{uncer}$), suppose we show the ensemble of classifiers several kinds of input. (1) We give input that all classifiers understand and yield the exact prediction scores. Consequently, classifiers are confident about their prediction scores, and the $total_{uncer}$ is minimum. (2) We show input that all classifiers understand and generate identical predictions but high entropy distribution over outcomes; then, classifiers are uncertain with high $\sigma$. (3) We show the ensemble something none of the classifiers understand; hence, all classifiers yield different prediction scores because the input comes from a very far region from the training data. Thus, the ensemble is very diverse with high entropy because we average various probability distributions together, then classifiers are uncertain with high $\rho$.

	\begin{equation}
	total_{uncer} = Entropy (avg_{pred})
        % gain(c_{id}, T_{i=1}) = cost(c_{id}, T_0)  - cost(c_{id}, T_{i=1})
        \label{eq:tuncer2}
    \end{equation}

In addition to the ensemble model that estimates $avg_{pred}$ and $total_{uncer}$ in the training phase, we train a causal model to measure the $CATE$. In particular, we utilize an \textit{orthogonal random forest (ORF)} algorithm because it reasonably deals with high-dimensional variable spaces. Thus, it is beneficial since the process execution logs have numerous event attributes with categorical values.% that could result in feature explosion.

Estimating the $CATE$ means we evaluate the difference between the probability of a negative outcome if we intervene and if we do not intervene. The higher the differences, the stronger the effect of the intervention. For explanation, we recall the motivating example in Sect.~\ref{sec:mex}, where the goal was to improve the performance of a loan origination process by raising the number of successful applications. Accordingly, we would give customers who are likely to decline the first offer another offer in a way that affects the probability of declining the first offer positively. Then we estimate what would happen for the probability of negative outcome when we send customers a second offer and when we do not. 
%To estimate CATE using ORF, the input needs to be in the form of $input = \{(T_i, Y_i, W_i, X_i)\}_{i=1}^n$ for $n$ instances. For each instance $i$, $T_i$ is the accepted treatment. $Y_i$ refers to the observed outcome. $T_i$ and $Y_i$ come from the preprocessing step (see Sect. 3.1), and they might be differ from one process to another based on the process objective.


%developed in our previous work~\cite{shoush2021prescriptive} to measure the $CATE$. Then, we filter and rank negative cases in the testing phase to determine when to intervene to maximize a gain function.

%Then, in the testing phase, we filter and rank negative cases to determine when to intervene to maximize a gain function.

%Then, in the testing phase, we filter and rank negative cases to determine when to intervene so that an adjusted gain is maximized. 

%At this stage, we have the estimated probability of cases likely to end with adverse outcomes ($avg_{pred}$) in addition to the estimated total uncertainty ($total_{uncer}$). The next step is to use these estimates with intervention effect ($CATE$), which is quantified based on our recent work~\cite{shoush2021prescriptive}, to determine whether or not to treat a given case in the testing phase.


\subsection{Testing Phase}

We first use the trained ensemble and causal models to obtain $avg_{pred}$, $total_{uncer}$, and $CATE$ scores for ongoing cases. Then, we use these scores to \textit{filter} ongoing cases into candidate ones and \textit{rank} them to choose the most profitable case to maximize \textit{a gain} function. We consider that resources are bounded and compare ongoing cases' current and future state scores. 
%We first \textit{filter} ongoing cases into candidate ones. Then \textit{rank} candidate cases to choose the most profitable to maximize \textit{an adjusted gain}. We consider that resources are bounded and compare ongoing cases' current and future state. 

%The testing phase introduces \textit{filtering} and \textit{scoring} techniques to choose the most profitable case among all potential cases to maximize an \textit{adjusted gain} considering that resources are bounded and comparing the selected case's current and future state.

\subsubsection{Filtering}

At run time, new events of ongoing cases keep coming continuously, and we first collate them via \textit{a prefix collator} to accumulate the sequence of events. Thus, at any point in time, we could have one or multiple ongoing cases that we choose from which one is the most profitable to trigger the intervention. Hence, ongoing cases need to be filtered to minimize the search space.

%During run time, new events for ongoing cases keep coming continuously, and we first collate them via \textit{a prefix collator} to accumulate the sequence of events. Accordingly, at any point in time, we could have one or multiple ongoing cases that we need to decide or choose which case is the most profitable one to utilize the intervention. Hence, filtering ongoing cases is crucial to reducing the search space. 

We use $avg_{pred}$, $total_{uncer}$, and $CATE$ scores to filter ongoing cases into candidate ones. The essence of these scores varies from one to another. The $avg_{pred}$ gives information about whether ongoing cases are likely to end negatively or not. At the same time, the $total_{uncer}$ shows how sure the model is with its predictions. It ranges from $0$ to $1$, where the predictive model is entirely certain or uncertain, respectively. Moreover, the $CATE$ is crucial to any PrPM technique, representing the expected impact of utilizing intervention on an ongoing case, e.g., when $CATE$ is above $0$, it impacts positively. 

%. It gives information about the expected impact of utilizing intervention on an ongoing case.%It gives information about the expected effect of utilizing intervention on an ongoing case at its current execution state.

%We ought to consider several factors when doing the filtration step. These factors mainly depend on the estimates from the trained models during the training phase, i.e., the estimated probability $(avg_{pred})$, the total uncertainty $(total_{uncer})$, and the $CATE$ in addition to a so-called \textit{intervention constraint} (hereafter $IC$). Based on these factors, as a first step, we decide if an ongoing case is eligible to be a candidate or potential case in its current state to retain it in further steps or not. 

%The essence of these factors mentioned above varies from one to another. On the one hand, the estimated probability gives information about whether ongoing cases end with a negative outcome or not. At the same time, the total uncertainty provides knowledge about how much we can trust and rely on the estimated probability.

%On the other hand, the $CATE$ is crucial to any PrPM technique. It gives information about the expected effect of utilizing intervention on an ongoing case at its current execution state. Finally, the intervention constraint is critical where intervention could be triggered and utilized under certain conditions. For example, based on our motivation example, sending customers a second offer is not feasible if they did not obtain the first one. 

%All the noted factors above are vital to determining candidate cases that later we define the best among them. However, two other aspects are critical to defining the best case that we discuss in the following subsections. 

All the abovementioned scores ($avg_{proba}$, $total_{uncer}$, $CATE$) are vital to determining candidate cases from which we will choose the most profitable. However, there are two other critical aspects to determine when to intervene and to define the most profitable case; how the estimated scores will change in the following state and whether resources are available or not.

%factors to define the most profitable case; how the estimated scores will change in the following state and whether resources are available or not. % to perform the intervention or not. 


%\subsubsection{Current and Future Process Execution State Analysis. }
\subsubsection{Future state scores estimation}
Considering only the current state scores of ongoing cases regardless of investigating what would occur in the future could be misleading. Because if we decide not to intervene, maybe it will be more effective to achieve higher gain when we utilize the intervention later than now, or we will be more sure about the prediction of the outcome and decide not to intervene at all. So, discovering what will happen in the future of ongoing cases allows deciding whether to intervene now or later. %So discovering what will happen at the future state of ongoing cases allow deciding whether to intervene now or later. 

%Considering only the current execution state of ongoing cases, regardless of exploring what would occur in the future, could be misleading. Because if we decide not to intervene, maybe it will be more effective to achieve higher gain when we utilize the intervention later than now, or we will be more sure about the prediction of the outcome and decide not to intervene at all. So discovering the future state of ongoing cases lets us know more or help us to decide whether to intervene now or later. 

To estimate what will happen in the future state, we predict the $avg_{pred}$, $CATE$, and $total_{uncer}$ in the future. So for each score, we will have two values: one representing the current state ($c\_avg_{pred}$, $c\_CATE$, $c\_total_{uncer}$) and the other representing the future ($f\_avg_{pred}$,  $f\_CATE$, $f\_total_{uncer}$). We follow a technique inspired by the \textit{k-nearest neighbors (KNN)}~\cite{peterson2009k} algorithm to get scores representing the future state, given the degree of \textit{similarity} and \textit{frequency}. 

%To estimate what will happen in the future state, we predict the probability of adverse outcomes $(avg_{pred})$, $CATE$, $total_{uncer}$ in the future state. So for each measure, we will have two values: one representing the current state and the other representing the future state ($c\_avg_{pred}$, $f\_avg_{pred}$, $c\_CATE$, $f\_CATE$, $c\_total_{uncer}$, $f\_total_{uncer}$). We follow a method motivated by the k-nearest neighbors (KNN) algorithm to get prediction scores that represent the future state. 

%First and for a given ongoing case at a particular prefix length ($k$), 

We look at previous cases similar to the ongoing one at the next prefix. For example, in a given case at prefix $4$, we want to know what will happen at prefix $5$. Then, we capture similar prefixes and define an aggregate score, i.e., the \textit{weighted average}. We consider the degree of \textit{similarity} using Euclidean distance to the current prefix, their \textit{frequency} because higher frequency means more weight and the scores for all similar prefixes. Accordingly, scores representing the future state ($f\_avg_{pred}$,  $f\_CATE$, $f\_total_{uncer}$) of ongoing cases are the weighted average from similar previous prefixes. The next step is to use current and future estimates to rank candidate cases and select the most profitable. 

%After estimating the prediction score ($avg_{proba}$), causal effect ($CATE$), and the prediction uncertainty ($total_{uncer}$) in the current and future states, we show how to use them to pick the most profitable case to allocate resources and trigger an intervention so that a gain function is maximized.
%After estimating the $avg_{pred}$, $CATE$, and $total_{uncer}$ in the current and future states, we show how to use them to pick the most profitable case to allocate resources and trigger an intervention so that an adjusted gain is maximized.
%We estimated the probability of unfavorable outcomes, CATE, and the total uncertainty at the current and future state of ongoing cases at this stage. The next step is to define how to use these estimates to define the best case to allocate resources and trigger an intervention in a way that maximizes an \textit{adjusted gain}.

%\subsubsection{Ranking and Resource Allocator.}
\subsubsection{Rank and retrieve the best case.}
%At the filtering step, we introduced three scores that have been assessed at the current and future states to filter ongoing cases into candidates. In contrast, the ranking discusses determining the most profitable case among all candidate cases to maximize a gain function.
%At the filtering step, we introduced three scores that have been assessed at the current and future states of ongoing cases. In contrast, the ranking discusses determining the most profitable case to maximize \textit{an adjusted gain} among all candidate cases. 

To define the most profitable case, we first distinguish between \textit{gain} and \textit{adjusted gain}. The \textit{gain} is the benefits we attain at one state only, either current or future, and it means we estimate two gains, one for the current state ($c\_gain$) and the other for the future state ($f\_gain$). In contrast, the \textit{adjusted gain} ($adj_{gain}$) is the benefits we attain considering current and future states. We use the $adj_{gain}$ as a decision function to determine whether to intervene now or later.


%At the filtration step, we introduced several factors to get potential or candidate cases and assess the current and future state estimates (the probability of unfavorable outcomes, CATE, and the total uncertainty) of ongoing cases execution. The scoring step discusses selecting the best case among all candidate cases to maximize an \textit{adjusted gain}. 

Triggering interventions may come with benefits and, at the same time, comes at a cost. The costs can vary from one process to another. However, for a given case $c_{id}$, there is generally a cost for applying the intervention ($cost(c_{id}, T_{i=1})$)) when $T=1$ and not applying the intervention ($cost(c_{id}, T_{i=0})$) when $T=0$. 

%We developed these costs and the corresponding \textit{gain} in our previous work~\cite{shoush2021prescriptive}. We recite them here to explain the adjusted gain to define when to intervene. 
%Triggering interventions may come with benefits and, at the same time, comes at a cost. The costs can vary from one process to another, but for a given case $c_{id}$, there is generally a cost for applying the intervention ($cost(c_{id}, T_{i=1})$)) when $T=1$ and not applying the intervention ($cost(c_{id}, T_{i=0})$) when $T=0$. We developed these costs and the corresponding \textit{gain} in our previous work~\cite{shoush2021prescriptive}. We recite them here to explain the adjusted gain to define when to intervene. 

%To define the \textit{adjusted gain}, we first describe the \textit{gain} we achieve from utilizing intervention on ongoing cases. However, triggering intervention may come with gain and, at the same time, comes at a cost. The costs can vary from one process to another, but for a given case $c_{id}$, there is generally a cost for applying the intervention ($cost(c_{id}, T_{i=1})$)) when $T=1$ and not applying the intervention ($cost(c_{id}, T_{i=0})$) when $T=0$. We described these costs and the corresponding \textit{gain} in our previous work~\cite{shoush2021prescriptive}. We recite them here to explain the adjusted gain.

The cost of not applying the intervention describes how much we lose if the negative outcome occurs, and it relies on the $avg_{pred}$ and cost of negative outcomes ($c_{uout}$), as shown in Eq.~\ref{eq:cnt}. In contrast, the cost of utilizing the intervention refers to how much we decrease the probability of negative outcomes considering the intervention cost ($c_{T_1}$), see Eq.~\ref{eq:ct}, which assumes $CATE$ is reliable. Costs are mainly identified via domain knowledge; however, we assume that the $c_{T_1}$ is less than the $c_{uout}$ to obtain meaningful results. 

%The cost of not applying the intervention relies on the $avg_{pred}$ and cost of negative outcomes ($c_{uout}$), as shown in Eq.~\ref{eq:cnt}. In contrast, the cost of utilizing the intervention contains the $CATE$, intervention cost ($c_{T_1}$), and $avg_{pred}$ and $c_{uout}$, see Eq.~\ref{eq:ct}.

	\begin{equation}
        cost(c_{id}, T_{i=0}) = avg_{pred} * c_{uout}
        \label{eq:cnt}
    \end{equation}
	\begin{equation}
        cost(c_{id}, T_{i=1}) = (avg_{pred} - CATE_1) * c_{uout} + c_{T_1}
        \label{eq:ct}
    \end{equation}
    
The corresponding gain ($gain(c_{id}, T_{i=1})$) from utilizing the intervention on $c_{id}$ is the benefits that allow the highest cost reduction in Eq.~\ref{eq:gain}

%based on Eqs.~\ref{eq:cnt} and~\ref{eq:ct}.

%The corresponding \textit{gain} ($gain(c_{id}, T_{i=1})$) from utilizing intervention $T=1$ on $c_{id}$ enables the highest cost reduction based on Eqs.~\ref{eq:cnt} and \ref{eq:ct}.

% The corresponding gain ($gain(c_{id}, T_{i=1})$) from utilizing intervention $T=1$ on $c_{id}$ enables the highest cost reduction between using and not using the intervention, as shown in Eq. \ref{eq:gain}.

	\begin{equation}
        gain(c_{id}, T_{i=1}) = cost(c_{id}, T_0)  - cost(c_{id}, T_{i=1})
        \label{eq:gain}
    \end{equation}
    
    
%After defining the \textit{gain} in general, we distinguish between the gain at the current state ($c\_gain(c_{id}, T_{i=1})$) and the gain at the future state ($f\_gain(c_{id}, T_{i=1})$). Thus, we estimate the costs of applying and not applying the intervention at both states, as shown in Eqs.~\ref{eq:ccnt}, \ref{eq:cct}, \ref{eq:fcnt} and \ref{eq:fct}. 


%After defining the gain in general, we now distinguish between the gain we achieve at a given case's current or future state. We estimate the costs of applying and not applying the intervention at both states, as shown in Eqs.~\ref{eq:ccnt}, \ref{eq:cct}, \ref{eq:fcnt}, and \ref{eq:fct}. 

% \begin{equation}
%         c\_cost(c_{id}, T_{i=0}) = c\_avg_{pred} * c_{uout}
%         \label{eq:ccnt}
%     \end{equation}
% 	\begin{equation}
%         c\_cost(c_{id}, T_{i=1}) = (c\_avg_{pred} - c\_CATE_1) * c_{uout} + c_{T_1}
%         \label{eq:cct}
%     \end{equation}
    
% \begin{equation}
%         f\_cost(c_{id}, T_{i=0}) = f\_avg_{pred} * c_{uout}
%         \label{eq:fcnt}
%     \end{equation}
% 	\begin{equation}
%         f\_cost(c_{id}, T_{i=1}) = (f\_avg_{pred} - f\_CATE_1) * c_{uout} + c_{T_1}
%         \label{eq:fct}
%     \end{equation}

We estimate the current state gain ($c\_gain(c_{id}, T_{i=1})$) using scores from the ensemble and causal models, see Eq.~\ref{eq:cgain}. In contrast, the gain for the future state ($f\_gain(c_{id}, T_{i=1})$) is based on the weighted average scores from previous similar prefixes, see Eq.~\ref{eq:fgain}.


%Then the gain is determined based on the current and future scores for candidate cases' current ($c\_gain(c_{id}, T_{i=1})$) and future ($c\_gain(c_{id}, T_{i=1})$) states, respectively, as shown in Eqs~\ref{eq:cgain} and~\ref{eq:fgain}.

%At this point, we have two gains, representing the current ($c\_gain(c_{id}, T_{i=1})$) and the future c gains in Eqs. \ref{eq:cgain} and \ref{eq:fgain}. %Next, we define the adjusted gain.
	\begin{equation}
        c\_gain(c_{id}, T_{i=1}) = c\_cost(c_{id}, T_0)  - c\_cost(c_{id}, T_{i=1})
        \label{eq:cgain}
    \end{equation}
    	\begin{equation}
        f\_gain(c_{id}, T_{i=1}) = f\_cost(c_{id}, T_0)  - f\_cost(c_{id}, T_{i=1})
        \label{eq:fgain}
    \end{equation}
    
Determining the gain for candidate cases' current and future states is vital to define the adjusted gain. To explain the adjusted gain, we first define \textit{an opportunity cost} that measures what we lose when choosing between two or more alternatives—for example, utilizing the intervention now or later. The opportunity cost ($opp_{cost}$) is the difference between the gain we could achieve in the future state of a given case and the gain in the current state, as shown in Eq.~\ref{eq:oppc}.

%We define an \textit{opportunity cost} that measures what we lose when choosing between two or more alternatives to identify the best case—for example, utilizing the intervention now or later. The opportunity cost ($opp_{cost}$) is the difference between the gain we could achieve in the future state of a given case and the gain at the current state, as shown in Eq. \ref{eq:oppc}.

	\begin{equation}
        opp_{cost} = f\_gain(c_{id}, T_{i=1})  - c\_gain(c_{id}, T_{i=1})
        \label{eq:oppc}
    \end{equation}

Given the opportunity cost, we define the \textit{adjusted gain} as the payoff (or gain) we acquire from utilizing the intervention on candidate cases considering current and future states. It is the difference between the $c\_gain(c_{id}, T_{i=1})$ and the $opp_{cost}$, as shown in Eq.~\ref{eq:again}. Thus, we define \textit{the most profitable case} as the one with the highest $adj_{gain}$, which means the lowest $opp_{cost}$.

%Given the opportunity cost, we introduce an \textit{adjusted gain} representing the payoff we achieve from utilizing intervention on candidate cases. We define the best case as the one with the highest adjusted gain ($adj_{gain}$), which means the minimum opportunity cost, as shown in Eq. \ref{eq:again}.

	\begin{equation}
        adj_{gain} = c\_gain(c_{id}, T_{i=1})  - opp_{cost}
        \label{eq:again}
    \end{equation}

\begin{table}[hbpt]
\centering

\caption{An example of defining gain.}
	\label{tab:againex}
\begin{tabular}{cccccl}
\hline
$c_{id}$ \hspace{0.3cm} & $c\_gain(c_{id}, T_{i=1})$ \hspace{0.3cm} & $f\_gain(c_{id}, T_{i=1})$ \hspace{0.3cm} & $opp_{cost}$ \hspace{0.3cm} & adju \hspace{0.3cm} & \multicolumn{1}{c}{decision} \\ \hline
A   & 7     & 12     & 5   & 3    & Wait                         \\
B   & 5    & 1    & -4  & 9   & Treat                        \\
C   & 3     & 3     & 0   & 3    & Neutral     \\ \hline                
\end{tabular}
\end{table}

For example, suppose we filtered ongoing cases into three candidates (see Tab.~\ref{tab:againex}) eligible for the intervention. Also, there is an available resource to do the intervention; we need to choose which one is more suitable to intervene now or later. If we consider only the gain from the current state, we assign resources to $c_{id}=A$ and treat it now. However, If we think about the gain from the future state, we observe that later we can achieve more gain if we do not intervene and previously assigned resources to $c_{id}=A$ inaccurately. Hence, it is more beneficial to allocate resources to $c_{id}=B$ and apply the intervention now since we might lose current gain later. Thus, using the adjusted gain to decide when to intervene could enhance the performance of PrPM.



Selecting the best or most profitable case can be judged efficiently based on the adjusted gain to maximize the total gain. However, triggering interventions as often as we want and immediately is impossible since resources are bounded in practice, which is the last aspect we need to consider.

\subsubsection{Resource Allocator.}
Monitoring resources and assigning them to cases that need intervention is critical. The resource allocator checks the availability of resources. Once the most profitable case is selected and a free resource is available, we assign that resource to the selected case and block it for a certain time, i.e., \textit{treatment duration} ($T_{dur}$).  The number of available resources and the time required to perform the intervention could be identified via domain knowledge~\cite{shoush2021prescriptive}. 
 %Once we have an available resource and a selected best case, we allocate that resource to that case to apply the intervention and block it for $T_{dur}$.  

% Choosing the best case can be judged efficiently based on the \textit{adjusted gain} and selecting the most profitable case to trigger the intervention. However, triggering interventions as often as we want and immediately is impossible since resources are bounded in practice which is the last factor we need to consider in our approach. Monitoring resources and assigning them to perform the intervention is critical, and we discussed it in our previous work\cite{shoush2021prescriptive}. Accordingly, we use it again in this approach. 

% We monitor all available resources we have, and once we have a selected best case with the highest adjusted gain, we assign resources to apply the intervention. Another dimension discussed in our previous work is how long we allocate resources to utilize the intervention, defined as the treatment duration ($T_{dur}$).

% Another dimension discussed in our previous work is how long we allocate resources to utilize the intervention that we defined as the treatment duration ($T_{dur}$).

==> BPM22_shoush/BG_and_RW.tex <==
\section{Background and Related Work} \label{sec:bgrw}

%Several PrPM techniques have been proposed, which can generally be unfolded into two main phases: $(1)$ A predictive process monitoring phase to estimate the probability of cases ending with unfavorable outcomes. $(2)$ A prescriptive phase in which interventions are prescribed, and their impact is estimated. In the following subsections, we illustrate these phases and detail recent related work.  

%Several PrPM techniques have been proposed, which can generally be unfolded into two main parts: \textit{Predictive process monitoring}, to estimate the probability of cases ending with unfavorable outcomes, and \textit{prescriptive process monitoring}, in which we move one step further after predictions to prescribe interventions and estimate its impact on negative cases. In the following subsections, we illustrate these parts and detail recent related work. 

\subsection{Predictive process monitoring}
Predictive process monitoring (PPM)~\cite{maggi2014predictive} is a complementary set of process mining methods to predict how ongoing cases will end. A PPM technique may, for instance, predict the remaining time for an ongoing case to be executed entirely~\cite{verenich2019survey}, the following action or activity to be executed~\cite{pauwels2021incremental}, or the outcome w.r.t group of outcomes, e.g., positive or negative~\cite{teinemaa2019outcome}. This paper focuses on the latter technique, known as an \textit{outcome-oriented} PPM.


%Predictive process monitoring (PPM) is a family of approaches that estimate how an ongoing case will complete. A PPM technique may, for instance, predicts the remaining time for running cases~\cite{verenich2019survey}, the next activity to be carried out~\cite{pauwels2021incremental}, or the final outcome w.r.t group of outcomes, e.g., positive and negative~\cite{teinemaa2019outcome}. This paper focuses on the latter class, known as \textit{an outcome-oriented } PPM.

% Predictive process monitoring (PPM) is a family of approaches that estimate how an ongoing case will complete. A PPM technique may, for instance, predict the remaining time for running cases~\cite{weytjens2021learning} or the next activity to be carried out~\cite{pauwels2021incremental} or the final outcome w.r.t group of outcomes, e.g., positive and negative~\cite{teinemaa2019outcome}. This paper focuses on the latter class that is called outcome-oriented PPM.

Recent outcome-oriented PPM methods estimate the prediction scores, i.e., probability of negative outcomes, for ongoing cases and classify them positively or negatively. If the prediction scores exceed a threshold, e.g., above $0.5$, the ongoing case is considered more likely to end negatively. 

However, outcome-oriented PPM methods focus only on making predictions as accurate as possible, regardless of the quality of the predictions. These methods rely on several \textit{case bucketing techniques}~\cite{di2016clustering}, e.g., a single bucket where cases are made in the same bucket and train one ML algorithm instead of several. Also, they rely on various \textit{feature encoding} techniques~\cite{teinemaa2019outcome} to map each case into a feature vector to train the ML algorithm. For instance, an aggregate encoding in which all events from the beginning of the case are considered. Thus, several aggregate functions may be used to the values an event has carried throughout the case.  Also, a handful of possible \textit{inter-case} features are extracted~\cite{kim2022encoding} to enrich the training of ML or deep learning (DL) algorithms~\cite{kratsch2021machine}. Still, these techniques aim to improve the performance of the prediction scores and ignore quantifying the prediction quality via measuring \textit{prediction uncertainty}.


%However, outcome-oriented PPM methods focus only on making predictions as accurate as possible, regardless of the quality of the predictions. These methods rely on several \textit{case bucketing techniques}~\cite{di2016clustering}, e.g., a single bucket where cases are made in the same bucket, and \textit{feature encoding} techniques~\cite{teinemaa2019outcome}, e.g., an aggregate method that maps each case into a feature vector. Additionally, they extract \textit{inter-case} features~\cite{kim2022encoding} to extract as much information from the event log to train a predictive model using classical ML or deep learning (DL) algorithms~\cite{kratsch2021machine}. Still, these techniques aim to improve the prediction scores performance and ignore quantifying the predictions’ quality via measuring \textit{prediction uncertainty}.

%Nevertheless, these techniques aim to improve the prediction’s performance and ignore quantifying the predictions’ quality via measuring the \textit{prediction uncertainty}.



%Recent outcome-oriented PPM methods focus only on making predictions as accurate as possible, regardless of the quality of the predictions. These methods rely on several \textit{case bucketing techniques}~\cite{di2016clustering}, e.g., a single bucket where cases are made in the same bucket, and \textit{feature encoding} techniques~\cite{teinemaa2019outcome}, e.g., an aggregate method that maps each case into a feature vector. Additionally,  they extract \textit{inter-case} features~\cite{kim2022encoding} to extract as much information from the event log to train a predictive model using classical ML or deep learning (DL) algorithms~\cite{kratsch2021machine}. However, these methods assume only the prediction's performance and ignore quantifying the predictions' quality via measuring the \textit{predictive uncertainty}.


% Recent outcome-oriented PPM methods focus only on making predictions as accurate as possible regardless of the quality of the predictions. These methods rely on several trace bucketing~\cite{di2016clustering}, feature encoding techniques~\cite{teinemaa2019outcome}, and inter-case features~\cite{kim2022encoding} to extract as much information from the event log to train a predictive model using classical machine learning or deep learning algorithms~\cite{kratsch2021machine}. 

%%%%%%Our work develops an outcome-oriented approach to get accurate predictions and measure uncertainty in a model's predictions to avoid expensive blunders in numerous industries and high-risk applications. 


% In our work, we develop an outcome-oriented approach to get accurate predictions, in addition, to measuring uncertainty in a model's predictions to avoid expensive blunders in numerous industries and high-risk applications. 

To the best of our knowledge, only one work from the literature considers estimating the model's prediction uncertainty explicitly, tackling another PPM task, i.e.,  remaining time~\cite{weytjens2021learning}. They learn the prediction uncertainty with artificial neural networks and a Monte Carlo (MC)~\cite{gal2016dropout} dropout technique that is unreliable for \textit{out-of-distribution} data (i.e., where there is an input case from a region very far from the trained data) and computationally expensive~\cite{abdar2021review}. 

%Another work by 
Metzger et al.~\cite{metzger2020triggering} introduces an approach to measure  the reliability of prediction scores using an ensemble of DL classifiers at different process states. This approach does not discuss the estimation of the prediction uncertainty ignoring the situation of out-of-distribution input. Moreover, where predictive models provide several prediction scores for the same input, i.e., \textit{outcomes overlap}.


%an approach to measure the reliability of predictions based on an ensemble of DL classifiers at different states in the process. This approach ignores the situation where an out-of-distribution input or outcomes overlap.  


% Only one work from the literature considers estimating the model's prediction uncertainty explicitly, tackling another PPM task, i.e.,  remaining time~\cite{weytjens2021learning}. They used Bayesian neural networks with the Monte Carlo (MC) dropout technique~\cite{gal2016dropout} that is unreliable for out-of-distribution data and computationally expensive~\cite{abdar2021review}.

% Another work by Metzger et al~\cite{metzger2020triggering}. introduces an approach to measure the reliability of predictions based on an ensemble of deep learning classifiers at different states in the process. This approach ignores the situation where an out-of-distribution input or classes overlap.  


\subsection{Prescriptive process monitoring}
Prescriptive process monitoring (PrPM) methods go beyond predictions to prescribe runtime interventions to prevent or mitigate negative outcome effects. These methods aim to improve the performance of business process executions by determining if and when to trigger an intervention to maximize a payoff.

Diverse PrPM methods have been proposed. Metzger et al.~\cite{metzger2020triggering} suggest using ongoing cases prediction scores and their reliability estimate with a reinforcement learning technique to discover when to trigger runtime interventions. Another work by Fahrenkrog et al.~\cite{fahrenkrog2021fire} proposes triggering one or more alarms when cases are more likely to end negatively, followed by an intervention. 

Both the work of Metzger et al. and that of Fahrenkrog et al. identify cases that need intervention. They assume that resources are unbounded and consider only the current state of a given case to determine when to intervene. Instead, we study the tradeoff between intervening now or later based on the current and future prediction scores. Thus, we identify the most profitable case and assign resources to it, considering that resources are limited.
%Both the work of Metzger et al. and that of Fahrenkrog et al. identify cases that need intervention, assume that resources are unbounded, and consider only the current state of a given case to determine when to intervene. Instead, we study the tradeoff between intervening now or later based on the current and future prediction scores and identify the most profitable case and assign resources to it, considering that resources are limited.
%Both the work of Metzger et al. and that of Fahrenkrog et al. identify cases that need intervention, assume that resources are unbounded, and consider only the current state of a given case. Instead, we compare the current and future states to select the best cases to utilize intervention and at the same time achieve maximal benefits, taking into account that resources are limited. 

Weinzerl et al.~\cite{weinzierl2020prescriptive} suggest a PrPM method to recommend the next best activity from a list of possible activities with a higher preference for a pre-defined KPI. Khan et al.~\cite{kratsch2021machine} introduce a memory-augmented neural net approach to recommend the most suitable path (meaning a set of activities until the completion of the process) based on pre-specified KPIs. Both the work of Weinzerl et al. and that of Khan et al. do not discuss an exact idea of interventions or when to trigger them to maximize payoff.

%do not discuss an exact idea of interventions and when to trigger them to maximize profit.


% Both the work of Weinzerl et al. and that of Khan et al. do not discuss an exact idea of intervention. Hence, it does not consider intervention influence and cost and the reality that intervention can only be initiated if resources are available to execute it. 

\subsection{Causal Inference}

%Causal Inference (CI)~\cite{xu2020causality} is a set of methods to predict what would occur if we adjust the process during its execution time by finding a cause-effect relationship between two variables, i.e., a feature and an outcome.

Causal Inference (CI)~\cite{xu2020causality} is a set of methods to predict what would occur if we adjust the process during its execution time by finding a cause-effect relationship between two variables, i.e., an intervention ($T$) and an outcome (Y). 

CI methods mainly unfold into two categories~\cite{guo2020survey}. The first category is \textit{structural causal models (SCMs)}, a multivariate statistical analysis method exploring structural relationships between dependent and independent variables. It depends mainly on discovering and building a causal graph by domain experts. 

%The second category is known as \textit{potential outcome frameworks} (aka the Neyman-Rubin Causal Model), a statistical analysis method that does not require a pre-built causal graph as the SCMs and relies on the concept of potential outcomes. We use this category in this paper to automatically estimate the causal effect (or \textit{conditional average treatment effect (CATE)}) of utilizing intervention on negative cases instead of manually building causal graphs. 

The second category is \textit{potential outcome frameworks} (a.k.a., the Neyman-Rubin Causal Model). A statistical analysis method that does not require a pre-built causal graph like the SCMs and relies on the concept of potential outcomes. We use this category in this paper to automatically estimate the causal effect (or \textit{conditional average treatment effect (CATE)}) of intervention on negative cases instead of manually building causal graphs.

For example, in a loan-origination process, a customer would have a loan if he received an \textit{intervention (T)}, e.g., a follow-up call three days after receiving the first offer; otherwise, he would have a different \textit{outcome (Y)}, e.g., offer declined. Accordingly, to measure the $CATE$ of having a follow-up call, we need to compare $Y$ for the same customer when receiving the follow-up call, i.e., $T=1$, and not receiving the follow-up call, i.e., $T=0$.

%CI methods mainly unfold into two categories~\cite{guo2020survey}, (1) Structural Causal Models (SCMs), a multivariate statistical analysis method exploring structural relationships between dependent and independent variables. It depends mainly on building a causal graph by domain experts. (2) Potential outcome frameworks (aka the Neyman-Rubin Causal Model), a statistical analysis method that does not require a pre-built causal graph as the previous method and relies on the concept of potential outcomes. For instance, in a loan-origination process, a customer would have a loan if he received a follow-up call (or a treatment: (T)) three days after receiving the first offer. In contrast, he would have a different outcome (Y: declines the offer) if he did not receive the follow-up call. To measure the effect of having a follow-up call, we need to compare the outcome for the same customer in both alternative ends. We use the latter approach from our recent work~\cite{shoush2021prescriptive}, which automatically focuses on estimating the treatment effect from observational data (hereafter called conditional average treatment effect (CATE)).


%SCMs have been introduced into process mining, particularly in~\cite{vanroot}, where authors examine whether a causal relation exists between a feature and an outcome. After that, they extended their work to include a counterfactual explanation to show why specific outcomes occur at the level of case prediction~\cite{qafari2021case}. Both studies~\cite{vanroot,qafari2021case} do not estimate the effect of utilizing intervention nor consider resource boundary.

Recent work uses the potential outcome method to estimate the $CATE$ of utilizing interventions. Specifically, in~\cite{bozorgi2021prescriptive}, the Authors introduce a PrPM technique to measure the effect of intervention at an individual case level to reduce the cycle time of the process.  It targets another PPM problem and considers only one process execution state; it also assumes that resources are unbounded.%This work targets another PPM problem, considers only one process execution state and assumes that resources are unbounded.

In our previous work~\cite{shoush2021prescriptive}, we propose a PrPM method that utilizes the potential outcome method and a resource allocator technique in the outcome-oriented PPM to allocate resources to cases with max gain. That work considers only a given case’s current state and triggers interventions when the prediction score and the causal effect exceed a threshold. However, we did not discuss the tradeoff between triggering an intervention now, given the level of uncertainty of the underlying predictive models versus later.

%We propose in our previous work~\cite{shoush2021prescriptive} a PrPM method that utilizes the potential outcome method and a resource allocator technique in the outcome-oriented PPM to allocate resources to cases with max gain. That work assumes only a given case’s current state and triggers interventions when the prediction score and the intervention effect exceed a threshold. However, the previous work does not discuss when to intervene, or discuss intervening now versus later.% to maximize the total gain.

%given the prediction uncertainty or postponing the intervention to a later state.

%Our previous work~\cite{shoush2021prescriptive} uses the potential outcome method and a resource allocator technique in the outcome-oriented PPM to allocate resources to cases with max gain. That work deals with only one state of the process execution and does not consider the quality of the predictive model predictions. 

% More recent work uses potential outcome techniques to estimate the impact of utilizing interventions. Specifically, in~\cite{bozorgi2021prescriptive}, the authors introduced a PrPM technique to measure the impact of intervention at an individual case level to reduce the cycle time of the process, which is another target problem. This work considers only one process execution state and assumes that resources are unbounded. 

% In our recent work~\cite{shoush2021prescriptive}, we use the potential outcome method in addition to a resource allocator technique in the outcome-oriented PPM task to allocate resources to cases that have max payoff from utilizing intervention. That work deals with only one state of the process execution and does not consider the quality of the predictive model predictions. 

% \subsection{Prescriptive phase}
% \subsubsection{Causal estimates}
% \subsubsection{Resource alloocator}

==> BPM22_shoush/Conclusion.tex <==
\section{Conclusion and Future Work} \label{sec:conclusion}

We presented a prescriptive monitoring method to determine if and when an intervention should be triggered on ongoing cases to maximize a gain function. The method leverages an ensemble model to estimate the probability of negative case outcomes and the associated prediction uncertainty. They are combined with a causal model to assess the effect of an intervention on the case outcome. These estimates and a filtering and ranking method are embedded in a resource allocator. It assigns resources to perform interventions to maximize total gain, considering the tradeoff between intervening now or later. An initial evaluation shows that taking into account the possible future states of ongoing cases and the level of prediction uncertainty leads to a higher gain than baselines that rely only on the current state of each case.

The proposed prescriptive method does not include constraints on when an intervention may be triggered. In practice, it is often not possible to trigger an intervention at any point in a case. For example, sending a second loan offer to a customer who has already accepted an offer at another bank is counter-productive. A direction for future work is to extend the approach with temporal rules on the interventions and  consider these rules in the intervention policy.


The proposed method is limited to handling one type of intervention. Also, an intervention is applied at most once to a case. Lifting these restrictions is another direction for future work. 





%We proposed a PrPM method to determine if and when an intervention is triggered on ongoing cases to maximize a cost function. The method adjusts an ensemble model to estimate the probability of cases likely to end negatively and the predictive uncertainty attached to its predictions, in combination with a causal model to assess the intervention effect of an intervention on cases' outcomes. These estimates with a filtering and ranking method are embedded in a resource allocator that assigns resources to perform interventions to maximize a total gain, considering the tradeoff between intervening now or later. An initial evaluation argues that investigating what will happen in the future state of ongoing cases, taking into account the level of uncertainty, enhances the efficiency of PrPM methods more than baseline methods. 


%In the proposed method, there are no constraints about the time we trigger the intervention. However, adding intervention constraints is critical in such an application. For example, sending another offer to a customer who has already accepted or declined the offer wastes resources and time, resulting in less gain. An avenue for future work is to consider the intervention constraints during the filtering step to ensure that cases are eligible to be treated to maximize payoff.  


\medskip\noindent\textbf{Reproducibility.} The implementation and source code of the method, together with instructions to reproduce the evaluation, can be found at:  \url{https://github.com/mshoush/prescriptive-monitoring-uncertainty}.


==> BPM22_shoush/Evaluation.tex <==
\section{Evaluation} \label{sec:evaluation}
To verify the effectiveness and relevance of the proposed method, we experimentally investigate whether we can learn when to trigger an intervention to maximize the total gain at the run time, considering the tradeoff between intervening now or later. We compare our results to baselines that consider either predictive models without quantifying the prediction uncertainty~\cite{fahrenkrog2021fire,metzger2020triggering} or only the current case's execution state scores~\cite{shoush2021prescriptive,bozorgi2021prescriptive} as state-of-the-art baselines by addressing the following research questions:  

%To verify the effectiveness and relevance of our proposed method, we experimentally investigate whether we can learn when to trigger an intervention to maximize an adjusted gain at run time. We also compare our results to several baselines that consider either a purely predictive approach~\cite{fahrenkrog2021fire} or only one case's execution state~\cite{shoush2021prescriptive,metzger2020triggering,bozorgi2021prescriptive} as state-of-the-art baselines by addressing the following research questions:  

    \begin{questions}
        \item To what extent does taking into account the current uncertainty prediction enhance the total gain?\label{rq:rq1}
        
        \item To what extent does taking into account the derivative of the uncertainty prediction and the adjusted gain enhance the total gain?\label{rq:rq2}
        %\item Considering the current state only of ongoing cases, to what extent does adding the total uncertainty to the filtering step enhance the total gain?\label{rq:rq1}
        %\item Assessing current and future states of ongoing cases, to what extent does the total adjusted gain evolve versus the current state only?\label{rq:rq2}
    \end{questions}
    
\subsection{Dataset}

We use a real-life event log, named \emph{BPIC2017}\footnote{\url{https://doi.org/10.4121/uuid:5f3067df-f10b-45da-b98b-86ae4c7a310b}}, publicly available from the 4TU.ResearchData. The log describes the execution of a loan origination process, and we choose this log for several reasons. First, it contains a clear notion for outcome definition and interventions utilized to show our method's efficiency. Second, this log contains $31,413$ applications and $1,202,267$ events, which is large enough and frequently used for predictive and prescriptive methods. %Accordingly, we rely on it to compare our proposed approach to other related work.

The \textit{BPIC2017} log is characterized by various case and event attributes, and we include all of them in our experiments. Additionally, we extracted other essential critical features in our work, such as the number of sent offers, event number, and additional temporal features. 



We used all original and extracted attributes as input for ensemble and causal models in the preprocessing step. Then we defined case outcomes based on the end state of cases, i.e., \textit{“A\_Pending”} state means positive outcome and \textit{“A\_canceled} or \textit{A\_Denied”} means negative outcome. After that, we defined the intervention that positively impacts the negative outcome as sending a second offer (or \textit{"Creat\_Offer"} activity) to all customers who received only one offer. Accordingly, we denoted cases with $T = 1$ based on the number of offers sent to each, i.e., cases that receive only one offer. Then, we extracted length prefixes no more than the $90^{th}$ percentile for each case to avoid bias from lengthy cases. Finally, we used an \textit{aggregate encoding} to encode the extracted prefixes.% in a feature vector ($X$).

%In the preprocessing step, we used all original and extracted attributes as input for ensemble and causal models. Then we defined case outcomes (\textit{positive or negative}) and cases that need intervention (\textit{send a second offer}) based on the end state of the case and the number of offers sent to each case as we did in our recent work~\cite{shoush2021prescriptive}. After that, we extracted length prefixes no more than the $90^{th}$ percentile for each case in the log to avert bias from lengthy cases. Finally, we used \textit{an aggregate encoding} technique to encode the extracted prefixes and not to lose information into a fixed-size feature vector. 

\subsection{Experimental Setup}
The experiments show our method's effectiveness during operation time with two main objectives: deciding when to intervene, either now or later, and selecting the most profitable case among all candidates to maximize the \textit{total gain}.

%The experiments show our approach's effectiveness during operation time with two main objectives: deciding whether to intervene, either now or later, and selecting the most profitable case among all candidates to maximize the $adj_{gain}$.

%Our experiments are designed to show our approach's effectiveness during operation time with two main objectives: deciding when to intervene, either now or later, and selecting the most profitable one among all candidate cases to maximize the adjusted gain.

% The experimental setup contains the implementation of our technique to discuss \ref{rq:rq1} and \ref{rq:rq2}, including code to train and evaluate the ensemble model, filtration, and scoring methods at run time and causal and resource allocation techniques from our recent work~\cite{shoush2021prescriptive}.
We adapted an ensemble model based on a \textit{Gradient Boosting Decision Tree (GBDT)} method to estimate the $avg_{pred}$ and $total_{uncer}$. In particular, we used  \textit{Catboost}~\cite{prokhorenkova2018catboost}, an open-source GBDT library with several tools to quantify the prediction uncertainty and automatically handle categorical features.


%We adapted an ensemble model using a \textit{Gradient Boosting Decision Tree (GBDT)} method to estimate the probability of undesired outcomes ($avg_{pred}$) and its total uncertainty ($total_{uncer}$), i.e., the entropy of average prediction. We used \textit{Catboost}~\cite{prokhorenkova2018catboost} because it is an open-source GBDT library and has several tools to quantify the predictive uncertainty.

\textit{Catboost} is trained with a \textit{negative log-likelihood} loss and \textit{Langevin optimization}~\cite{ustimenko2021sglb} to ensure global conversion instead of a local optimum and generate an ensemble of several independent GBDT. Additionally, we used the following parameters during training: ensemble size of $50$, a learning rate of $0.05$, a subsample of $0.82$, and a max tree depth of $12$.

Catboost returns a probability distribution over the case outcomes. This
distribution is based on a given model version, i.e., on the seed used to initialize the model parameters before training. So we train the same model using different seed initialization and evaluating these models on the same input to obtain the $avg_{pred}$ and its $total_{uncer}$. We use an ORF algorithm implemented in the  \emph{EconMl}\footnote{\url{https://github.com/microsoft/EconML}} to train a causal model to estimate the CATE.

%We use an ORF algorithm to train a causal model to estimate the $CATE$ created in the  \emph{EconMl}\footnote{\url{https://github.com/microsoft/EconML}}.

%We use a causal model developed in our recent work~\cite{shoush2021prescriptive} to estimate the CATE, which uses an orthogonal random forest (ORF) created in the  \emph{EconMl}\footnote{\url{https://github.com/microsoft/EconML}}.

%We adapted a causal model developed in our recent work~\cite{shoush2021prescriptive} to estimate the $CATE$ that used an \textit{orthogonal random forest (ORF)} implemented in the \emph{EconMl}\footnote{\url{https://github.com/microsoft/EconML}} package.

%To estimate the $CATE$, we adapted a causal model developed in our recent work that used an \textit{orthogonal random forest (ORF)} implemented in the \emph{EconMl}\footnote{\url{https://github.com/microsoft/EconML}} package.

We follow the machine learning workflow to train both ensemble and causal models. We temporally split the data into training ($60\%$), validation ($20\%$ ), and testing ($20\%$) sets. Training and validation sets are used to train and tune model parameters, while the testing set is used to evaluate the model’s performance.% models performance. 
\begin{table}[hbpt]
%\vspace*{-7mm}
%\scriptsize
\centering
\caption{Parameter settings of the introduced method}
\label{tab:param}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccc}
\hline
$avg_{proba}$\hspace{0.5cm} & $CATE$\hspace{0.5cm}  & \hspace{0.5cm}$total_{uncer}$ & $\Delta total_{uncer} \hspace{0.5cm}$                                            & \hspace{0.5cm}\#resources \hspace{0.5cm} & \hspace{0.5cm} $c_{uout}$ \hspace{0.5cm}  \hspace{0.5cm}& $c_{T_1}$ \hspace{0.5cm}& $T_{dur}$  (sec)                                                                       \\ \hline
\textgreater $0.5$          & \textgreater $0$      & $< 0.25, 0.5, 0.75$ \hspace{1cm}     & $< 0, -0.5, -0.1, -0.15, -0.2, -0.25, -0.3$ \hspace{0.3cm} & $1, 2, ...10$ & $20$    & $1$   & \begin{tabular}[c]{@{}c@{}}Fixed = $60$\\  \hspace{0.8cm}Normal $\in$ \{$1, 60$\}\\ \hspace{1.4cm}  Exponential $\in$ \{$1, 60$\}\end{tabular}
\\ \hline
\end{tabular}}
\end{table}

During the testing time, we follow the configurations shown in Tab.~\ref{tab:param}. First, ongoing cases are filtered into candidates. We filter cases based on the estimated probability of $avg_{pred}$ \textgreater $0.5$ to ensure that cases are highly probable to end negatively and $CATE$ \textgreater $0$ to guarantee that intervention has a positive impact.%to guarantee that utilizing intervention on cases has a positive impact.

%with $avg_{proba}$ \textgreater $0.5$ has a positive impact. 

Additionally, we filter cases using the $total_{uncer}$ to see how sure the predictive model is with the predictions. The estimated $total_{uncer}$ ranges from $0$, where the model is certain, to $1$, which is entirely uncertain. We experiment with three thresholds (see Tab.~\ref{tab:param}) when considering only the current state of cases. 

%As shown in Table \ref{tab:param}, we experiment with several thresholds when we consider only the current state of ongoing cases. 
On the other hand, we use the $opp_{coast}$ or $adj_{gain}$ when we consider both current and future states of ongoing cases. At the same time, with and without a derivative of the total uncertainty ($\Delta total_{uncer}$), representing the difference between $c\_total_{uncer}$ and $f\_total_{uncer}$. Accordingly, we filter cases based on the $c\_avg_{pred}$ and $c\_CATE$ and then select the case with the highest $adj_{gain}$ with and without $\Delta total_{uncer}$ when it is below $0$ or negative values (see Table~\ref{tab:param}), which means the predictive model becomes more uncertain in the future state.

%On the other hand, when we consider both current and future states of ongoing cases, we use the $opp_{coast}$ or $adj_{gain}$ with and without a derivative of the prediction uncertainty ($\Delta total_{uncer}$), representing the difference between $c\_total_{uncer}$ and $f\_total_{uncer}$, to decide which case is the most profitable and when to trigger the intervention. Accordingly, we filter cases based on the $c\_avg_{pred}$ and $c\_CATE$ and then select the case with the highest $adj_{gain}$ with and without $\Delta total_{uncer}$ when it is below $0$ or negative values (see Table~\ref{tab:param}), which means the predictive model becomes more uncertain in the future state.

% or the case with the highest adjusted gain and ∆totaluncer is below zero or negative values values (see Table 2), which means the predictive model becomes more uncertain in the future state.

% On the other hand, when we consider both current and future states of ongoing cases, we use a derivative of the total uncertainty ($\Delta total_{uncer}$), representing the difference between $c\_total_{uncer}$ and $f\_total_{uncer}$. Accordingly, we include cases when $\Delta total_{uncer}$ is below zero or negative values (see Table~\ref{tab:param}), which means the predictive model becomes more uncertain in the future state. 

%is below a specific number, as shown in Table \ref{tab:param}.





%Finally, for the number of available resources, $c_{T_1}$ and $c_{uout}$, and the $T_{dur}$, we follow the same suggestions proposed in~\cite{shoush2021prescriptive}.

\subsection{Results}
We show results here based on one $T_{dur}$ distribution, i.e., fixed. Since the normal distribution achieves similar results to the fixed in terms of the total gain and is higher than the exponential distribution as the variability is higher in the latter. Also, we observed that the behavior for different thresholds for $total_{uncer}$ and $\Delta total_{uncer}$ is the same, i.e. when we lower the threshold, fewer cases are treated with no substantial effect on the total gain per case. Hence, we present results using one threshold, i.e., the higher value for $total_{uncer} < 0.75$ and $\Delta total_{uncer} < 0$. However, The full results of experimenting with all thresholds and $T_{dur}$ distributions are available in supplementary material~\footnote{\url{https://zenodo.org/record/6381445\#.YjwaFfexWuA}{\label{supp}}}.


%We show results here based on the fixed distribution for the $T_{dur}$ because it is similar to the normal distribution. Normal and fixed distributions achieve a higher total gain than exponential because the variability is higher in the exponential distribution. We also found that the behavior for different thresholds for $total_{uncer}$ and $\Delta total_{uncer}$ is the same, i.e., when we lower the threshold, fewer cases are treated with no substantial effect on the total gain per case. Accordingly, we show results based on only one threshold for the $total_{uncer}$ and $\Delta total_{uncer}$, $0.75$ and $0$, respectively. The full results of experimenting with all thresholds and $T_{dur}$ are available in the supplementary material\footnote{\url{https://zenodo.org/record/6381445#.YjwaFfexWuA}}.

To discuss~\ref{rq:rq1}, we consider only the current state scores of ongoing cases. Then, examine how the total gain evolves when adding the  current prediction uncertainty ($c\_total_{uncer}$) to the filtering step. Besides the estimated prediction score ($c\_avg_{proba}$ ) and the causal effect ($c\_CATE$). We compare this to baselines shown in~\cite{shoush2021prescriptive,bozorgi2020process}, where only the $avg_{proba}$ and $CATE$ are set, see Fig.~\ref{fig:rq1}.% in the filtering step.


%Fig.~\ref{fig:rq1} shows that adding the current uncertainty prediction does not improve the total gain unless the number of available resources is above $80\%$; otherwise, the baseline wins. However, when the number of resources increases, the baseline treats more cases with less total gain. In contrast, adding the current uncertainty prediction allows allocating resources efficiently since fewer cases are treated but with higher total gain than the baseline.

%We show the results in two steps. First, and to discuss~\ref{rq:rq1}, we consider only the current state scores of ongoing cases and examine how the total gain evolves when adding the current uncertainty prediction ($c\_total_{uncer}$) to the filtering step beside the estimated $c\_avg_{proba}$ and $c\_CATE$. We compare this step to baselines presented in~\cite{shoush2021prescriptive,bozorgi2020process}, where only the $avg_{proba}$ and $CATE$ are assessed, see Fig.~\ref{fig:rq1}.% in the filtering step.

%We compare this step to a baseline presented in~~\cite{shoush2021prescriptive}, where only the $c\_avg_{proba}$ and $c\_CATE$ are assessed.

%We compare this step to baselines presented in~\cite{shoush2021prescriptive,bozorgi2020process}, where only the $avg_{proba}$ and $CATE$ are assessed in the filtering step. We did not compare our method to a purely predictive method presented in~\cite{fahrenkrog2021fire,metzger2020triggering} because it is shown in~\cite{shoush2021prescriptive,bozorgi2020process}that considering the probability of negative outcomes only achieves less total gain than the situation where we consider predictive and causal models together. 

\begin{figure}[!h]
\centering
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=\linewidth, ]{images/RQ1.pdf}
  \scalebox{0.7}{\parbox{\linewidth}{%
  \caption{RQ1: Where $avgProba\_CATE$ means $c\_avg_{proba} > 0.5$ \& $c\_CATE > 0$. Also, $avgProba\_CATE\_tUncer$ means  $c\_avg_{proba} > 0.5$ \& $c\_CATE > 0$ \&  $c\_total_{uncer} < 0.75$.}
  \label{fig:rq1}}}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/RQ2.pdf}
  \scalebox{0.7}{\parbox{\linewidth}{%
  \caption{RQ2: Where $avgProba\_CATE\_oppCost$ refers to the $adj_{gain}$ is maximized. Also, $avgProba\_CATE\_oppCost\_dUncer$ refers to the $adj_{gain}$ is maximized \& $\Delta total_{uncer} <0$.}
  \label{fig:rq2}}}
\end{subfigure}
\caption{The total gain progress under the same number of available resources.}
\label{fig:res}
\end{figure}


The results in Fig.~\ref{fig:rq1} explain that adding the current prediction uncertainty improves the total gain when the available resources exceed 80\%. Also, the baseline treats more cases with less total gain (as shown in the supplementary~\ref{supp}). In contrast, adding the current prediction uncertainty allows efficient allocation of resources since fewer cases are treated but with a higher total gain than the baseline. Because considering the current prediction uncertainty does not trigger the intervention until the predictive model becomes more sure about its predictions and achieves higher total gain.

%Fig.~\ref{fig:rq1}  shows that adding the current uncertainty prediction does not improve the total gain unless the number of available resources is above $80\%$.However, when the number of resources increases, the baseline treats more cases with less total gain. In contrast, adding the current uncertainty prediction allows efficient allocation of resources since fewer cases are treated but with a higher total gain than the baseline. Because considering the current uncertainty prediction does not trigger the intervention until the predictive model becomes more sure about its predictions and achieves higher total gain.
%Then, and to answer~\ref{rq:rq2}, we consider two states of ongoing cases, i.e., current and future, to study how the total gain is improved when considering the $opp_{cost}$ and the $\Delta total_{uncer}$. 

Turning to discuss~\ref{rq:rq2}, we consider two states’ scores of ongoing cases, i.e., current and future, to estimate the $opp_{cost}$ and the $adj_{gain}$ and their impacts on the total gain. Hence, we decide when to intervene and allocate the available resources to ongoing cases based on two things: first, cases with the maximum $adj_{gain}$ only, and second, cases with the maximum $adj_{gain}$ and the $\Delta total_{uncer} <0$. We compare this method to the baseline in~\ref{rq:rq1} and consider the current prediction uncertainty only, see Fig.~\ref{fig:rq2}.

%Turning to discuss~\ref{rq:rq2}, we consider two states' scores of ongoing cases, i.e., current and future, to estimate the $opp_{cost}$ and the $adj_{gain}$ and their impacts on the total gain. Hence, we allocate resources to ongoing cases based on two things: first, cases with the maximum $adj_{gain}$, and second, cases with the maximum $adj_{gain}$ and the $\Delta total_{uncer} <0$. We compare this method to the~\ref{rq:rq2}, where we consider only the current state of ongoing cases, see Fig.~\ref{fig:rq2}.


The results in Fig.~\ref{fig:rq2} show that the total gain is highly affected by the trade off of current and future state scores under the same quantity of consumed resources. The proposed method achieves a significant improvement in terms of the total gain and outperforms the baselines (cf.~Fig \ref{fig:rq1}). We found that considering the $adj_{gain}$ as a decision function to determine when to intervene is more efficient than considering it with the $\Delta total_{uncer}$. Still, considering the derivative of the prediction uncertainty could achieve a higher gain when the available resources are below 10\%. Because when the number of available resources increases, more cases are treated without ensuring that the $total_{uncer}$ is sufficient.
%Fig.~\ref{fig:rq2} indicates that the total gain depends on the tradeoff of current and future state scores, under the same quantity of consumed resources. We observe that analyzing what will happen in the future state of ongoing cases highly affects the gain we achieve from utilizing interventions. Also, considering the $adj_{gain}$ as a method to decide when to intervene is more efficient than considering it with the $\Delta total_{uncer}$. 

%We show the results in two steps. First, and to discuss \ref{rq:rq1}, we consider only the current state of ongoing cases and examine how the \textit{total gain} evolves when we add the $total_{uncer}$ in the filtering step bediseds the $avg_{pred}$ and $CATE$. Then, and to answer \ref{rq:rq2}, we assume the current and future state of ongoing cases to study how the \textit{adjusted gain} is improved compared to the total gain in the previous step. Hence, we filter cases based on two things: first, the estimated $avg_{pred}$ and $CATE$, and second the $avg_{pred}$, $CATE$ and the $\Delta total_{uncer}$. 

%We compare our approach to three baselines. The first baseline is based on work proposed by~\cite{fahrenkrog2021fire,metzger2020triggering}. We compare our approach to a purely predictive model without assuming either the $total_{uncer}$ or $CATE$ in the filtration step and use $CATE$ as the gain acquired from applying intervention. The second baseline is presented in~\cite{shoush2021prescriptive,bozorgi2021prescriptive}, where the $avg_{pred}$ and $CATE$ are assessed without the $total_{uncer}$ to maximize the \textit{net gain}. The third baseline mainly compares how the \textit{adjusted gain} is enhanced compared to total gain when we consider ongoing cases' current and future state. 

The proposed PrPM method results in Fig.~\ref{fig:res} demonstrate a higher total gain than the baselines. Accordingly, estimating the prediction uncertainty of the underlying predictive model and analyzing the tradeoff between triggering an intervention now versus later based on the adjusted gain and the opportunity cost can optimize the performance of PrPM methods, hence, business processes.


%demonstrate a higher total gain than the baselines that do not consider quantifying the prediction uncertainty or the opportunity cost.  This implies that estimating the prediction uncertainty of the underlying predictive model and analyzing the tradeoff between triggering intervention now versus later based on the current and future state scores can improve the efficiency of PrPM methods.

%Based on the results shown in Fig.~\ref{fig:res}, the proposed method achieves a higher total gain than the baselines that do not consider quantifying the uncertainty or the opportunity cost. This implies that  estimating the uncertainty of predictive models predictions and analyzing the tradeoff between current and future states scores can improve the efficiency of PrPM methods. 

\subsection{Threats to Validity}
Our method's evaluation has an external validity threat (lack of generalizability) because of its dependence on only one dataset. Accordingly, the evaluation is vague and needs more experiments using other logs to be followed up.

We assume that $CATE$ is accurate and will reduce the probability of negative outcomes. Also, the intervention will be triggered only once for each ongoing case. Accordingly, there is a threat to ecological reality where cases may be treated more than once via multiple interventions. Moreover, the  $CATE$ may not represent the natural causal effect because of unobserved confounders.


The experiments’ setup used one feature encoding technique and did not discuss the selection bias of the causal model due to variables that affect both the outcome and the intervention. Utilizing other encoding and selection bias techniques is a hint for future work to improve the performance of PrPM methods.
%The experiments' setup used one feature encoding technique and did not discuss the selection bias of the causal model due to variables that affect both the outcome and the treatment. Adding other encoding and selection bias techniques is a direction for future work. 

==> BPM22_shoush/Introduction.tex <==
\section{Introduction} \label{sec:introduction}
\textit{Prescriptive Process monitoring (PrPM)} is a family of process mining methods that trigger runtime actions to optimize a process's performance~\cite{fahrenkrog2021fire,metzger2020triggering}. PrPM methods use \textit{event logs} describing past business process executions to train \textit{machine learning (ML)} algorithms for two goals. \textit{First,} the trained ML models predict how an instance of the process (a.k.a.\ case) will unfold. For example,  whether the case leads to a positive outcome (e.g., a customer is satisfied) or a negative outcome (e.g., a customer launches a complaint)~\cite{teinemaa2019outcome}. %Further, the trained ML models may predict the remaining time to complete a case~\cite{verenich2019survey} or the subsequent activity to be executed~\cite{pauwels2021incremental}. 
\textit{Second}, PrPM methods use ML to assess  the effect of triggering an action (herein called an \textit{intervention}) on the probability of a negative outcome or a performance measure.

%\textit{Prescriptive Process monitoring (PrPM)} is a family of process mining methods that trigger actions, at runtime, to optimize the performance of a process~\cite{fahrenkrog2021fire,metzger2020triggering}. PrPM methods use \textit{event logs}, representing past business process executions, to train \textit{machine learning (ML)} algorithms with two purposes. First, the trained ML models may predict how an instance of the process (a.k.a.\ case) will unfold, for example, will it lead to a positive or a negative outcome (a.k.a.\ outcome prediction~\cite{teinemaa2019outcome}), what is the remaining time to complete the case~\cite{verenich2019survey}, or what will be the next activity~\cite{pauwels2021incremental}?. Second, PrPM methods rely on ML models to estimate the effect of triggering an action (herein called an \textit{intervention}) on the probability of a negative outcome or on a performance measure.
%, e.g., in an order-to-cash process, the order is canceled or delivered improperly, indicating a problem that could be avoided.

%\textit{Prescriptive Process monitoring (PrPM)}~\cite{fahrenkrog2021fire,metzger2020triggering} is a complementary set of process mining techniques that help enterprises improve their business processes. PrPM takes a historical \textit{event log} to train machine learning (ML) algorithms with two main tasks: First, the predictive part, to predict what will happen for ongoing cases in the future from different aspects, such as outcome prediction, that we focus on in this work, remaining time, and subsequent action or activity prediction. Second, the prescriptive part, suppose the predicted outcome is undesired, e.g., customer dissatisfaction. In that case, PrPM methods recommend actions (aka \textit{interventions}) and decide when the process workers employ these interventions to preclude the impact of adverse outcomes.

Recently, various PrPM methods have been proposed~\cite{shoush2021prescriptive,fahrenkrog2021fire,metzger2020triggering,bozorgi2021prescriptive}. These methods, however, implement intervention policies based on predictions of negative outcomes without considering  the uncertainty of these predictions. Also, they  trigger an intervention when the predicted probability of a negative outcome is above a threshold, without considering potential increases or decreases in this predicted probability that may occur as the case unfolds further. Finally, these methods do not consider the fact that there are limited resources available to perform the recommended interventions.

%define when to trigger interventions based on prediction scores from the current state of ongoing cases only, ignoring expected improvements at the future state.


%These methods, however, trigger interventions when cases are likely to end undesirably, assuming that predictions will be continuously generated, even when wholly uncertain and regardless of the consequences of lower quality predictions. Moreover, they only define gains from using interventions at the current state of an ongoing case, ignoring expected changes at the future state.

%Several PrPM methods have been introduced recently~\cite{fahrenkrog2021fire,metzger2020triggering,bozorgi2021prescriptive}. These approaches lack different things: First and w.r.t the predictive part, they assume that predictions will be continuously generated, even when wholly uncertain and regardless of the consequences of lower quality predictions. Second and w.r.t the prescriptive part, they only assume profits from utilizing interventions at the current case state, ignoring expected changes at the following state. Finally, they assume that resources to apply interventions are unbounded, and the interventions can be triggered many times at any point.  

In this paper, we address the following problem: Given a set of cases, and given a type of intervention that generally decreases the likelihood of a negative case outcome. \textit{How do we select the cases for which applying the intervention (now or later) maximizes a gain function, considering the available resources to perform interventions?} Here, the gain function considers the tradeoff between the cost of applying the intervention to a case and the cost of negative outcomes.
% the opportunity cost, and the causal effect of applying interventions. 

%In this paper, we tackle the following problem: \textit{Given a set of cases ending with undesired results and an intervention that mostly decreases the likelihood of adverse outcomes, how to pick the suitable case to assign the limited resources to it and perform the intervention to maximize an adjusted gain?} Here, the adjusted gain considers the costs of intervention, cases ending in negative results, and the opportunity cost. 

To address this problem, we first apply an ensemble-based predictive model to estimate the negative outcome probability for each case, and we estimate the associated uncertainty. Using a causal model, we then determine the causal effect of applying an intervention on the negative outcome probability. We then use the negative outcome probability, the uncertainty, and the estimated causal effect and apply a \textit{filtering} and \textit{ranking} mechanism to identify cases for which an intervention would be most profitable (highest gain). We also consider the tradeoff (i.e., opportunity cost) between triggering an intervention in the current state, given the level of uncertainty of the predictive model, versus postponing the intervention to a later state. The paper reports an empirical evaluation comparing the proposed approach against state-of-the-art baselines.

%We then determine the causal effect of applying an intervention on the negative outcome probability using a causal model. Using the negative outcome probability, the uncertainty, and the estimated causal effect, we then apply a \textit{filtering} and a \textit{ranking} mechanism to identify the cases for which an intervention would be most profitable (highest gain). We also consider the tradeoff (i.e.\ opportunity loss) between triggering an intervention in the current state, given the level of uncertainty of the predictive model, versus postponing the intervention to a later state. The paper reports on an empirical evaluation that compares the proposed approach against state-of-the-art baselines.
%, which only consider the current state of the case’s execution~\cite{shoush2021prescriptive,bozorgi2020process,fahrenkrog2021fire,metzger2020triggering}.



%To address this problem, we first adjust an \textit{ensemble-based} predictive model to estimate the uncertainties aligned with the probabilities of negative outcomes. We then determine the \textit{causal effect} of utilizing the intervention on negative cases generated by a causal model developed in our previous work~\cite{shoush2021prescriptive}. Moreover, we introduce a \textit{filtering and ranking} technique to identify the most profitable case based on the current and future case's state, considering the availability of resources. We report on assessing a real-life dataset to compare the proposed method with state-of-the-art baselines, which only consider the current state of the case's execution~\cite{shoush2021prescriptive,bozorgi2020process,fahrenkrog2021fire,metzger2020triggering}.% or rely on a purely predictive model~\cite{fahrenkrog2021fire,metzger2020triggering}.


%To address this problem, in the beginning, we adapted an ensemble-based predictive model to estimate the uncertainties aligned with the probabilities of adverse outcomes and a causal effect estimation method to measure the impact of utilizing the intervention on negative cases. Then, we introduce a filtering and scoring technique to identify the most suitable case based on the current and following case's state, considering the availability of resources. We evaluated our proposed approach using one real-life event log. 

The following section motivates the proposed method. Sect.~\ref{sec:bgrw} then presents background concepts and related work. Sect.~\ref{sec:approach} explains the proposed method, while Sect.~\ref{sec:evaluation} discusses the empirical evaluation. Finally, Sect.~\ref{sec:conclusion} concludes and discusses future work directions.



%\textit{Predictive process monitoring} (PPM) is a complementary set of process mining techniques designed to help enterprises daily. PPM takes a historical event log to train a machine learning (ML) algorithm to predict what will happen for ongoing cases in the future from different aspects, such as outcome prediction~\cite{teinemaa2019outcome}, which we focus on in this work, remaining time prediction~\cite{weytjens2021learning}, and subsequent action prediction~\cite{pauwels2021incremental}. 

%Recent \textit{outcome-oriented} prediction methods continuously produce predictions, even when wholly uncertain and nevertheless of the influences. Accordingly, estimating the two types of uncertainty~\cite{malinin2020uncertainty} (\textit{data uncertainty}, when cases' outcomes overlap, and \textit{knowledge uncertainty}, when cases are out of distribution) is vital to distinguish between higher and lower quality predictions.  Additionally, the ignorance of uncertainty is a significant barrier to their adoption in practice. 



==> BPM22_shoush/motivation_ex.tex <==
\section{Motivating Example} \label{sec:mex}
In \textit{a loan origination process}, a case starts when a customer submits his documents to obtain a loan. Then a process worker (or an employee) verifies the submitted documents. When they are valid, the employee sends an offer to the customer via different channels, such as phone calls or emails. This case ends positively when the customer accepts the offer and receives the loan, or negatively when the customer declines the offer or the employee rejects the application.

The principal concern arises when cases end negatively, leading to less payoff. One way to deal with this could be to predict negative cases based on prediction scores.  Then trigger an alarm to take a proactive action or an intervention, e.g., \textit{making a follow-up call}, when the prediction score exceeds a certain threshold. %However, this strategy could be ineffective.
%The main problem occurs when applications end negatively. One way to deal with this could be to predict unsuccessful applications then trigger an alarm to take a proactive action or an intervention, e.g., making a follow-up call. However, this strategy could be ineffective. 

However, this strategy could be ineffective. Suppose an intervention policy where interventions are triggered to cases that are likely to end negatively based on low-quality prediction scores. Also, all employees are occupied and cannot immediately perform the intervention for all cases. Additionally, triggering interventions without considering their effect could be misleading since they may provide low or negative impact when utilized.

A more proper method is to quantify the prediction uncertainty to estimate how sure predictive models are with the prediction scores. Moreover, measuring the causal effect of utilizing interventions and considering the availability of resources. Another step that may enhance the overall payoff could be considering the tradeoff between triggering interventions now versus postponing them for a later state. In this paper, we discuss this method and evaluate its performance.%We discuss this method in this paper and evaluate its performance.% on PrPM. 
%Suppose the situation where interventions are triggered to applications that are likely to end negatively based on low-quality predictions or where all workers are busy and cannot apply the intervention immediately or even after performing it, gives low or negative impact. A more appropriate procedure is to quantify predictions quality via measuring the uncertainty, the causal effect of utilizing interventions, and  considering the availability of resources. All this could be done at the current and future application states for a given case and compare both states' scores to maximize payoff. We discuss the latter approach in this paper. 


% Regarding a \textit{loan origination process}, at the beginning of this process execution, customers apply or submit application documents to acquire a loan at the end. The process workers (or employees) check and verify the submitted documents then send offers to clients through different channels such as phone calls or emails. Then clients either accept or decline the sent offer where the application ends successfully or unsuccessfully. 

% The principal issue is when applications end with undesired outcomes where customers decline the offer or employees cancel the application. One way to avoid this could be to predict unsuccessful applications (or cases) and trigger an alarm to take proactive action or intervention, e.g., making a follow-up call. However, this strategy could be useless. 

% Suppose the case of triggering interventions to cases that are likely to end with negative results based on low-quality predictions or where all workers are busy so that cannot immediately apply the intervention to all negative cases. Also, where utilizing intervention on cases with no positive effect. A more appropriate strategy is to consider the quality of predictions, the effect of utilizing interventions, and the availability of resources at the current state of the process execution and also at the following state. We discuss the latter approach in this work. 

